Segmentation Assisted Incremental Test Time Adaptation in an Open World

In dynamic environments, unfamiliar objects and distribution shifts are often encountered, which challenge the generalization abilities of the deployed trained models. This work addresses Incremental Test Time Adaptation of Vision Language Models, tackling scenarios where unseen classes and unseen domains continuously appear during testing. Unlike traditional Test Time Adaptation approaches, where the test stream comes only from a predefined set of classes, our framework allows models to adapt simultaneously to both covariate and label shifts, actively incorporating new classes as they emerge. Towards this goal, we establish a new benchmark for ITTA, integrating single image TTA methods for VLMs with active labeling techniques that query an oracle for samples potentially representing unseen classes during test time. We propose a segmentation assisted active labeling module, termed SegAssist, which is training free and repurposes the segmentation capabilities of VLMs to refine active sample selection, prioritizing samples likely to belong to unseen classes. Extensive experiments on several benchmark datasets demonstrate the potential of SegAssist to enhance the performance of VLMs in real world scenarios, where continuous adaptation to emerging data is essential. Project-page:https://manogna-s.github.io/segassist/

==> sec/main_results.tex <==
\newcommand{\detailedTableImageNetRADomainnNetClipart}{
\begin{table*}[]
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lccccccccccccc}
\toprule

& \multirow{2}{*}{Method} & \multicolumn{4}{c}{ImageNet-R} & \multicolumn{4}{c}{ImageNet-A} & \multicolumn{4}{c}{DN-Clipart}\\
\cmidrule(r){3-6} \cmidrule(r){7-10} \cmidrule(r){11-14}
&  & $Acc_{k} \uparrow$ & $Acc_{u} \uparrow$ &  HM$\uparrow$ & ICDD $\downarrow$ & $Acc_{k} \uparrow$ & $Acc_{u} \uparrow$ &  HM$\uparrow$ & ICDD $\downarrow$  & $Acc_{k} \uparrow$ & $Acc_{u} \uparrow$ &  HM$\uparrow$ & ICDD $\downarrow$  \\ \midrule
\multirow{5}{*}{\rotatebox{90}{ZS-Eval}}  & Random    & 76.39 & 36.69 & 49.57 & 0.2590 & 52.02 & 15.26 & 23.60 & 0.4533 & 72.46 & 18.37 & 29.31 & 0.4496 \\
                                        ~ & MSP       & 76.98 & 53.20 & 62.92 & 0.1721 & 52.24 & 16.08 & 24.59 & 0.4189 & 72.94 & 27.97 & 40.44 & 0.3640 \\
                                        ~ & Entropy   & 77.21 & 48.91 & 59.89 & 0.2199 & 52.41 & 13.22 & 21.11 & 0.4383 & 73.05 & 28.04 & 40.52 & 0.3418 \\
                                        ~ & Margin    & 76.77 & 50.38 & 60.84 & 0.1638 & 52.48 & 12.40 & 20.06 & 0.4579 & 72.87 & 25.10 & 37.34 & 0.3909 \\
\cmidrule(r){2-14}
                                        ~ & SegAssist & 76.99 & 54.83 & 64.05 & 0.1601 & 52.24 & 15.53 & 23.94 & 0.4147 & 72.94 & 27.66 & 40.11 & 0.3671 \\
\midrule
\multirow{5}{*}{\rotatebox{90}{TDA}}      & Random & 80.20 & 39.95 & 53.33 & 0.2590 & 55.19 & 17.51 & 26.58 & 0.4533 & 74.67 & 18.92 & 30.19 & 0.4496 \\
                                        ~ & MSP & 80.53 & 62.50 & 70.38 & 0.1325 & 55.75 & 11.65 & 19.27 & 0.4393 & 75.20 & 32.41 & 45.30 & 0.3587 \\
                                        ~ & Entropy  & 80.67 & 53.12 & 64.06 & 0.1952 & 55.84 & 12.19 & 20.02 & 0.4495 & 75.36 & 28.35 & 41.20 & 0.3632 \\
                                        ~ & Margin  & 80.30 & 54.38 & 64.85 & 0.1647 & 55.86 & 13.28 & 21.46 & 0.4727 & 75.11 & 31.42 & 44.31 & 0.3703 \\
\cmidrule(r){2-14}
                                        ~ & SegAssist & 80.53 & 62.66 & 70.48 & 0.1307 & 55.75 & 11.65 & 19.27 & 0.4393 & 75.15 & 32.45 & 45.32 & 0.3526 \\
\midrule
\multirow{5}{*}{\rotatebox{90}{DPE}}      & Random & 79.47 & 41.94 & 54.90 & 0.2590 & 54.26 & 19.35 & 28.52 & 0.5788 & 75.10 & 19.84 & 31.39 & 0.4496 \\
                                        ~ & MSP & 80.05 & 59.24 & 68.09 & 0.1964 & 54.84 & 15.87 & 24.62 & 0.5788 & 75.63 & 30.67 & 43.64 & 0.3623 \\
                                        ~ & Entropy  & 80.75 & 0.10 & 0.19 & 0.5605 & 54.97 & 2.32 & 4.44 & 0.5788 & 75.47 & 2.70 & 5.21 & 0.5501 \\
                                        ~ & Margin  & 79.75 & 55.53 & 65.47 & 0.1712 & 54.62 & 21.39 & 30.74 & 0.4624 & 75.09 & 29.23 & 42.09 & 0.3764 \\
\cmidrule(r){2-14}
                                        ~ & SegAssist & 79.99 & 61.28 & 69.39 & 0.1638 & 54.43 & 24.11 & 33.42 & 0.5788 & 75.69 & 30.64 & 43.62 & 0.3722 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{ITTA Results: ImageNet-R, ImageNet-A, DN-Clipart}
\end{table*}
}

\newcommand{\detailedTableDomainnNetPaintingSketchInfograph}{
\begin{table*}[]
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lccccccccccccc}
\toprule

& \multirow{2}{*}{Method} & \multicolumn{4}{c}{DN-Painting} & \multicolumn{4}{c}{DN-Sketch} & \multicolumn{4}{c}{DN-Infograph}\\
\cmidrule(r){3-6} \cmidrule(r){7-10} \cmidrule(r){11-14}
&  & $Acc_{k} \uparrow$ & $Acc_{u} \uparrow$ &  HM$\uparrow$ & ICDD $\downarrow$ & $Acc_{k} \uparrow$ & $Acc_{u} \uparrow$ &  HM$\uparrow$ & ICDD $\downarrow$  & $Acc_{k} \uparrow$ & $Acc_{u} \uparrow$ &  HM$\uparrow$ & ICDD $\downarrow$  \\ \midrule
\multirow{5}{*}{\rotatebox{90}{ZS-Eval}} & Random & 67.64 & 27.80 & 39.41 & 0.3804 & 65.07 & 24.83 & 35.94 & 0.4021 & 48.61 & 14.25 & 22.04 & 0.4571 \\
        ~ & MSP & 67.91 & 37.40 & 48.24 & 0.3091 & 65.46 & 36.81 & 47.13 & 0.3264 & 49.02 & 22.53 & 30.87 & 0.4377 \\
        ~ & Entropy  & 68.04 & 35.97 & 47.06 & 0.3566 & 65.42 & 33.40 & 44.22 & 0.3585 & 49.33 & 16.63 & 24.88 & 0.4678 \\
        ~ & Margin  & 67.87 & 33.67 & 45.01 & 0.3586 & 65.41 & 31.30 & 42.34 & 0.3647 & 49.00 & 22.00 & 30.36 & 0.3973 \\
\cmidrule(r){2-14}
        ~ & SegAssist & 67.93 & 39.49 & 49.95 & 0.3028 & 65.40 & 38.59 & 48.54 & 0.3066 & 49.04 & 22.53 & 30.88 & 0.4337 \\
\midrule
\multirow{5}{*}{\rotatebox{90}{TDA}} & Random & 71.87 & 31.91 & 44.20 & 0.3804 & 68.16 & 26.65 & 38.32 & 0.4021 & 55.65 & 16.56 & 25.53 & 0.4571 \\
        ~ & MSP & 72.17 & 37.32 & 49.20 & 0.3518 & 68.38 & 41.26 & 51.47 & 0.3193 & 55.98 & 25.27 & 34.82 & 0.4191 \\
        ~ & Entropy  & 72.27 & 36.48 & 48.49 & 0.3584 & 68.52 & 31.60 & 43.26 & 0.3838 & 56.39 & 17.73 & 26.98 & 0.4545 \\
        ~ & Margin  & 72.21 & 39.98 & 51.47 & 0.3206 & 68.51 & 34.67 & 46.04 & 0.3520 & 55.98 & 22.71 & 32.31 & 0.4207 \\
\cmidrule(r){2-14}
        ~ & SegAssist & 72.15 & 40.95 & 52.25 & 0.3238 & 68.49 & 39.17 & 49.84 & 0.3316 & 55.95 & 26.62 & 36.07 & 0.4156 \\
\midrule
\multirow{5}{*}{\rotatebox{90}{DPE}} & Random & 71.10 & 34.34 & 46.31 & 0.3804 & 68.08 & 28.40 & 40.08 & 0.5689 & 53.31 & 18.48 & 27.44 & 0.4571 \\
        ~ & MSP & 71.39 & 43.86 & 54.34 & 0.3259 & 68.02 & 39.58 & 50.04 & 0.5689 & 53.49 & 29.99 & 38.44 & 0.3891 \\
        ~ & Entropy  & 71.71 & 1.10 & 2.16 & 0.5298 & 68.40 & 0.00 & 0.00 & 0.5689 & 53.74 & 0.14 & 0.28 & 0.5509 \\
        ~ & Margin  & 71.22 & 43.55 & 54.05 & 0.3075 & 68.22 & 37.76 & 48.61 & 0.3433 & 53.75 & 20.22 & 29.39 & 0.4432 \\
\cmidrule(r){2-14}
        ~ & SegAssist & 71.37 & 45.67 & 55.70 & 0.3037 & 68.02 & 39.88 & 50.28 & 0.3186 & 53.59 & 23.70 & 32.87 & 0.4201 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{ITTA Results: DN-Painting, Sketch, Infograph}
\end{table*}
}


\newcommand{\TableImageNetRADomainnNetClipart}{
\begin{table*}[]
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lccccccc}
\toprule

& \multirow{2}{*}{Method} & \multicolumn{2}{c}{ImageNet-R} & \multicolumn{2}{c}{ImageNet-A} & \multicolumn{2}{c}{DN-Clipart}\\
% \cmidrule(r){3-6} \cmidrule(r){7-10} \cmidrule(r){11-14}
&  & HM$\uparrow$ & ICDD $\downarrow$ & HM$\uparrow$ & ICDD $\downarrow$  &   HM$\uparrow$ & ICDD $\downarrow$  \\ \midrule
\multirow{5}{*}{\rotatebox{90}{ZS-Eval}}  & Random    & 49.57 & 0.2590 & 23.60 & 0.4533 & 29.31 & 0.4496 \\
                                        ~ & MSP       & 62.92 & 0.1721 & 24.59 & 0.4189 & 40.44 & 0.3640 \\
                                        ~ & Entropy   & 59.89 & 0.2199 & 21.11 & 0.4383 & 40.52 & 0.3418 \\
                                        ~ & Margin    & 60.84 & 0.1638 & 20.06 & 0.4579 & 37.34 & 0.3909 \\
                                        ~ & SegAssist & 64.05 & 0.1601 & 23.94 & 0.4147 & 40.40 & 0.3660 \\
% \cmidrule(r){2-14}
\midrule
\multirow{5}{*}{\rotatebox{90}{TDA}}      & Random      & 53.33 & 0.2590 & 26.58 & 0.4533 & 30.19 & 0.4496 \\
                                        ~ & MSP         & 70.38 & 0.1325 & 19.27 & 0.4393 & 45.30 & 0.3587 \\
                                        ~ & Entropy     & 64.06 & 0.1952 & 20.02 & 0.4495 & 41.20 & 0.3632 \\
                                        ~ & Margin      & 64.85 & 0.1647 & 21.46 & 0.4727 & 44.31 & 0.3703 \\
                                        ~ & SegAssist   & 70.48 & 0.1307 & 19.27 & 0.4393 & 45.52 & 0.3536 \\
% \cmidrule(r){2-14}
\midrule
\multirow{5}{*}{\rotatebox{90}{DPE}}      & Random      & 54.90 & 0.2590 & 28.52 & 0.5788 & 31.39 & 0.4496 \\
                                        ~ & MSP         & 68.09 & 0.1964 & 24.62 & 0.5788 & 43.64 & 0.3623 \\
                                        ~ & Entropy     & 0.19  & 0.5605 & 4.44  & 0.5788 & 5.21  & 0.5501 \\
                                        ~ & Margin      & 65.47 & 0.1712 & 30.74 & 0.4624 & 42.09 & 0.3764 \\
                                        ~ & SegAssist   & 69.39 & 0.1638 & 33.42 & 0.5788 & 44.06 & 0.3690 \\
% \cmidrule(r){2-14}
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{ITTA Results: ImageNet-R, ImageNet-A, DN-Clipart}
\end{table*}
}


\newcommand{\TableDomainnNetPaintingSketchInfograph}{
\begin{table*}[]
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lccccccccccccc}
\toprule

% & \multirow{2}{*}{Method} & \multicolumn{4}{c}{DN-Painting} & \multicolumn{4}{c}{DN-Sketch} & \multicolumn{4}{c}{DN-Infograph}\\
% \cmidrule(r){3-6} \cmidrule(r){7-10} \cmidrule(r){11-14}
% &  & $Acc_{k} \uparrow$ & $Acc_{u} \uparrow$ &  HM$\uparrow$ & ICDD $\downarrow$ & $Acc_{k} \uparrow$ & $Acc_{u} \uparrow$ &  HM$\uparrow$ & ICDD $\downarrow$  & $Acc_{k} \uparrow$ & $Acc_{u} \uparrow$ &  HM$\uparrow$ & ICDD $\downarrow$  \\ \midrule
\multirow{5}{*}{\rotatebox{90}{ZS-Eval}}  & Random      & 39.41 & 0.3804 & 35.94 & 0.4021 & 22.04 & 0.4571 \\
                                        ~ & MSP         & 48.24 & 0.3091 & 47.13 & 0.3264 & 30.87 & 0.4377 \\
                                        ~ & Entropy     & 47.06 & 0.3566 & 44.22 & 0.3585 & 24.88 & 0.4678 \\
                                        ~ & Margin      & 45.01 & 0.3586 & 42.34 & 0.3647 & 30.36 & 0.3973 \\
                                        ~ & SegAssist   & 49.95 & 0.3028 & 48.54 & 0.3066 & 30.88 & 0.4337 \\
        % \cmidrule(r){2-14}
\midrule
\multirow{5}{*}{\rotatebox{90}{TDA}}      & Random      & 44.20 & 0.3804 & 38.32 & 0.4021 & 25.53 & 0.4571 \\
                                        ~ & MSP         & 49.20 & 0.3518 & 51.47 & 0.3193 & 34.82 & 0.4191 \\
                                        ~ & Entropy     & 48.49 & 0.3584 & 43.26 & 0.3838 & 26.98 & 0.4545 \\
                                        ~ & Margin      & 51.47 & 0.3206 & 46.04 & 0.3520 & 32.31 & 0.4207 \\
                                        ~ & SegAssist   & 52.25 & 0.3238 & 49.84 & 0.3316 & 36.07 & 0.4156 \\
        % \cmidrule(r){2-14}
\midrule
\multirow{5}{*}{\rotatebox{90}{DPE}}      & Random      & 46.31 & 0.3804 & 40.08 & 0.5689 & 27.44 & 0.4571 \\
                                        ~ & MSP         & 54.34 & 0.3259 & 50.04 & 0.5689 & 38.44 & 0.3891 \\
                                        ~ & Entropy     & 02.16 & 0.5298 & 00.00 & 0.5689 & 00.28 & 0.5509 \\
                                        ~ & Margin      & 54.05 & 0.3075 & 48.61 & 0.3433 & 29.39 & 0.4432 \\
                                        ~ & SegAssist   & 55.70 & 0.3037 & 50.28 & 0.3186 & 32.87 & 0.4201 \\
        % \cmidrule(r){2-14}
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{ITTA Results: DN-Painting, Sketch, Infograph}
\end{table*}
}

\newcommand{\TableMainResultsHMICDD}{
\begin{table*}[]
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lccccccccccccc}
\toprule

& \multirow{2}{*}{Method} & \multicolumn{2}{c}{ImageNet-R} & \multicolumn{2}{c}{ImageNet-A} & \multicolumn{2}{c}{DN-Clipart} & \multicolumn{2}{c}{DN-Painting} & \multicolumn{2}{c}{DN-Sketch} & \multicolumn{2}{c}{DN-Real}\\
 \cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8} \cmidrule(r){9-10} \cmidrule(r){11-12} \cmidrule(r){13-14}
&  & HM$\uparrow$ & ICDD $\downarrow$ & HM$\uparrow$ & ICDD $\downarrow$  &   HM$\uparrow$ & ICDD $\downarrow$ & HM$\uparrow$ & ICDD $\downarrow$ & HM$\uparrow$ & ICDD $\downarrow$  &   HM$\uparrow$ & ICDD $\downarrow$  \\ \midrule
\multirow{5}{*}{\rotatebox{90}{ZS-Eval}}  & Random    & 49.57 & 0.2590 &          23.60 &         0.4533  & 29.31 & 0.4496 & 39.41 & 0.3804 & 35.94 & 0.4021 & 57.59 & 0.2988\\
                                        ~ & MSP       & 62.92 & 0.1721 & \textbf{24.59} & 0.4189 & \textbf{40.44} & \textbf{0.3640} & 48.24 & 0.3091 & 47.13 & 0.3264 & 75.86 & 0.1185\\
                                        ~ & Entropy   & 59.89 & 0.2199 &          21.11 &           0.4383 & 40.12 & 0.3688 & 47.06 & 0.3566 & 44.22 & 0.3585 & 66.05 & 0.2017\\
                                        ~ & Margin    & 60.84 & 0.1638 &          20.06 &           0.4579 & 37.34 & 0.3909 & 45.01 & 0.3586 & 42.34 & 0.3647 & 74.25 & 0.1319\\
     \cmidrule(r){2-14}
                                        ~ & SegAssist & \textbf{64.05} & \textbf{0.1601} & 23.94 & \textbf{0.4147} & 40.40 & 0.3660 & \textbf{49.95} & \textbf{0.3028} & \textbf{48.54} & \textbf{0.3066} & \textbf{75.93} & \textbf{0.1165}\\
\midrule
\multirow{5}{*}{\rotatebox{90}{TDA}}      & Random      & 53.33 & 0.2590 & 16.58 & 0.4433 & 30.19 & 0.4496 & 44.20 & 0.3804 & 38.32 & 0.4021 & 59.61 & 0.2988\\
                                        ~ & MSP         & 70.38 & 0.1325 & 19.27 & 0.4393 & 45.30 & 0.3587 & 49.20 & 0.3518 & \textbf{50.47} & \textbf{0.3193} & 75.46 & 0.1325\\
                                        ~ & Entropy     & 64.06 & 0.1952 & 20.02 & 0.4495 & 41.20 & 0.3632 & 48.49 & 0.3584 & 43.26 & 0.3838 & 63.49 & 0.2447\\
                                        ~ & Margin      & 64.85 & 0.1647 & \textbf{21.46} & 0.4427 & 44.31 & 0.3703 & 51.47 & 0.3256 & 46.04 & 0.3520 & 77.86 & 0.1183\\
 \cmidrule(r){2-14}
                                        ~ & SegAssist   & \textbf{70.48} & \textbf{0.1307} & 19.27 & \textbf{0.4393} & \textbf{45.52} &\textbf{ 0.3536} & \textbf{52.25} & \textbf{0.3238} & 49.84 & 0.3316 & \textbf{75.91} & \textbf{0.1284}\\
\midrule
\multirow{5}{*}{\rotatebox{90}{DPE}}      & Random      & 54.90 & 0.2590 & 28.52 & 0.4621 & 31.39 & 0.4496 & 46.31 & 0.3804 & 40.08 & 0.5689 & 60.46 & 0.2988\\
                                        ~ & MSP         & 68.09 & 0.1964 & 24.62 & 0.4718 & 43.64 & \textbf{0.3623} & 54.34 & 0.3259 & 50.04 & 0.5689 & \textbf{73.12} & \textbf{0.1779}\\
                                        ~ & Entropy     & 0.19  & 0.5605 & 4.44  & 0.5788 & 5.21  & 0.5501 & 02.16 & 0.5298 & 00.00 & 0.5689 & 5.28  & 0.5487 \\
                                        ~ & Margin      & 65.47 & 0.1712 & 30.74 & 0.4624 & 42.09 & 0.3764 & 54.05 & 0.3075 & 48.61 & 0.3433 & 71.93 & 0.2074\\
     \cmidrule(r){2-14}
                                        ~ & SegAssist   & \textbf{69.39} & \textbf{0.1638} & \textbf{33.42} & \textbf{0.4598} & \textbf{44.06} & 0.3690 & \textbf{55.70} & \textbf{0.3037} & \textbf{50.28} & \textbf{0.3186} & 73.04 & 0.1810\\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{ITTA Results: ImageNet-R, ImageNet-A, DN-Clipart, Painting, Sketch, Infograph}
\end{table*}
}
